FairGBM: Gradient Boosting with Fairness Constraints

Tabular data is prevalent in many high-stakes domains, such as financial services or public policy. Gradient Boosted Decision Trees (GBDT) are popular in these settings due to their scalability, performance, and low training cost. While fairness in these domains is a foremost concern, existing in-processing Fair ML methods are either incompatible with GBDT, or incur in significant performance losses while taking considerably longer to train. We present FairGBM, a dual ascent learning framework for training GBDT under fairness constraints, with little to no impact on predictive performance when compared to unconstrained GBDT. Since observational fairness metrics are non-differentiable, we propose smooth convex error rate proxies for common fairness criteria, enabling gradient-based optimization using a ``proxy-Lagrangian'' formulation. Our implementation shows an order of magnitude speedup in training time relative to related work, a pivotal aspect to foster the widespread adoption of FairGBM by real-world practitioners.

==> Notation/acronyms.tex <==
\acrodef{AI}{Artificial Intelligence}
\acrodef{AOF}{Account Opening Fraud}


\acrodef{DART}{Dropout meets Multiple Additive Regression Trees}
\acrodef{DL}{Deep Learning}

\acrodef{FP}{False Negative}
\acrodef{FNR}{False Negative Rate}

\acrodef{FP}{False Positive}
\acrodef{FPR}{False Positive Rate}
\acrodef{FWL}{Fair Weak Learning}

\acrodef{EFB}{Exclusive Feature Bundling}

\acrodef{GDPR}{General Data Protection Regulation}
\acrodef{GBDT}{Gradient Boosting Decision Tree}
\acrodef{GBM}{Gradient Boosting Machine}
\acrodef{GOSS}{Gradient-based One-Side Sampling}

\acrodef{LP}{Label Positive}
\acrodef{LN}{Label Negative}

\acrodef{MART}{Multiple Additive Regression Trees}

\acrodef{RM}{Random Massaging}
\acrodef{RR}{Random Relabeling} 

\acrodef{SDB}{Shift Decision Boundary}
\acrodef{SVM}{Support Vector Machine}

\acrodef{TFCO}{TensorFlow Constrained Optimization}
\acrodef{TN}{True Negative}
\acrodef{TNR}{True Negative Rate}

\acrodef{TP}{True Positive}
\acrodef{TPR}{True Positive Rate}

\acrodef{ML}{Machine Learning}


==> Notation/iclr2021_math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\newcommand{\euler}{e}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\suchthat}{s.t.}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables-2022/results_best_fair_models.tex <==
\begin{tabular}{lcccc}

\toprule
     \multirow{2}{*}{\textbf{Algo.}} & \multicolumn{2}{c}{\textbf{Validation}}       & \multicolumn{2}{c}{\textbf{Test}}            \\
     & \textbf{Pred. Perf.} & \textbf{Fairness} & \textbf{Pred. Perf.} & \textbf{Fairness} \\
\midrule
%^{\lozenge\blacklozenge}
  \multicolumn{5}{c}{ACSIncome} \\
\midrule
 FairGBM    & $1$ &  $1$ &  $1$ &  $1$ \\
 LightGBM   & $1$ &  $1$ &  $1$ &  $1$ \\
 GS         & $1$ &  $1$ &  $1$ &  $1$ \\
 RS         & $1$ &  $1$ &  $1$ &  $1$ \\
 EG         & $1$ &  $1$ &  $1$ &  $1$ \\
\midrule

  \multicolumn{5}{c}{AOF} \\
\midrule
 FairGBM    & $1$ &  $1$ &  $1$ &  $1$ \\
 LightGBM   & $1$ &  $1$ &  $1$ &  $1$ \\
 GS         & $1$ &  $1$ &  $1$ &  $1$ \\
 RS         & $1$ &  $1$ &  $1$ &  $1$ \\
\bottomrule
\\
\end{tabular}


==> tables-2022/results_best_tradeoff_models.tex <==
\begin{tabular}{l|cccc|cccc|cccc|cc}

\toprule
    \multirow{3}{*}{\textbf{Algorithm}} & \multicolumn{4}{c|}{\textbf{Trade-off} $\alpha = 0.5$} & \multicolumn{4}{c|}{\textbf{Trade-off} $\alpha = 0.75$} & \multicolumn{4}{c|}{\textbf{Trade-off} $\alpha = 0.95$} & \multicolumn{2}{|c}{\textbf{Run-time}} \\
        & \multicolumn{2}{c}{\textbf{Validation}}  & \multicolumn{2}{c|}{\textbf{Test}} & \multicolumn{2}{c}{\textbf{Validation}}  & \multicolumn{2}{c|}{\textbf{Test}} & \multicolumn{2}{c}{\textbf{Validation}}  & \multicolumn{2}{c|}{\textbf{Test}} & \multirow{2}{*}{\textbf{Total (h)}} & \multirow{2}{*}{\textbf{Relative}} \\
        & \textbf{Fair.} & \textbf{Perf.} & \textbf{Fair.} & \textbf{Perf.} & \textbf{Fair.} & \textbf{Perf.} & \textbf{Fair.} & \textbf{Perf.} & \textbf{Fair.} & \textbf{Perf.} & \textbf{Fair.} & \textbf{Perf.} &  &  \\
\midrule
  \multicolumn{15}{c}{ACSIncome dataset} \\
\midrule
 FairGBM    
    & $0.999$ & $0.817$ & $0.997$ & $0.817$ 
    & $0.999$ & $0.817$ & $0.997$ & $0.817$
    & $0.994$ & $0.817$ & $0.993$ & $0.818$
    & $9.9$ & x2.1 \\

 LightGBM   
    & $0.819$ & $0.792$ & $0.818$ & $0.792$ 
    & $0.776$ & $0.806$ & $0.774$ & $0.807$ 
    & $0.712$ & $0.820$ & $0.706$ & $0.820$
    & $4.6$ & \textit{baseline} \\

 GS         
    & $0.683$ & $0.819$ & $0.676$ & $0.820$ 
    & $0.683$ & $0.819$ & $0.676$ & $0.820$ 
    & $0.683$ & $0.819$ & $0.676$ & $0.820$
    & $43.8$ & x9.6 \\    %% > Fairlearn-GS-10x10 (Note: 10x10)

 RS         
    & $0.787$ & $0.812$ & $0.793$ & $0.812$ 
    & $0.787$ & $0.812$ & $0.793$ & $0.812$ 
    & $0.787$ & $0.812$ & $0.793$ & $0.812$
    & $37.1$ & x8.1 \\    %% > Fairlearn-GS (Note: 100x1)

 EG         
    & $0.949$ & $0.818$ & $0.939$ & $0.819$ 
    & $0.949$ & $0.818$ & $0.939$ & $0.819$ 
    & $0.949$ & $0.818$ & $0.939$ & $0.819$
    & $99.4$ & x21.7 \\    %% > Fairlearn-EG

\midrule

  \multicolumn{15}{c}{AOF dataset} \\
\midrule
 FairGBM    
    & $0.952$ & $0.655$ & $0.915$ & $0.666$
    & $0.904$ & $0.674$ & $0.876$ & $0.661$
    & $0.904$ & $0.674$ & $0.876$ & $0.661$
    & $3.5$ & x2.4 \\

 LightGBM   
    & $0.812$ & $0.519$ & $0.866$ & $0.526$ 
    & $0.635$ & $0.617$ & $0.774$ & $0.595$ 
    & $0.319$ & $0.682$ & $0.357$ & $0.672$
    & $1.4$ & \textit{baseline} \\

 GS         
    & $0.988$ & $0.277$ & $0.999$ & $0.284$ 
    & $0.988$ & $0.277$ & $0.999$ & $0.284$ 
    & $0.988$ & $0.277$ & $0.999$ & $0.284$
    & $21.4$ & x14.7 \\

 RS         
    & $0.922$ & $0.357$ & $0.935$ & $0.359$ 
    & $0.888$ & $0.381$ & $0.889$ & $0.389$ 
    & $0.377$ & $0.547$ & $0.336$ & $0.563$
    & $10.3$ & x7.1 \\

\bottomrule
\end{tabular}


==> tables-2022/results_bootstrapping_alpha=0.50.tex <==
\begin{tabular}{l|cccc}
\toprule
    \multirow{3}{*}{\textbf{Algorithm}} & \multicolumn{4}{c}{\textbf{Trade-off} $\alpha = 0.50$} \\
        & \multicolumn{2}{c}{\textbf{Validation}}  & \multicolumn{2}{c}{\textbf{Test}} \\
        & \textbf{Fair. (\%)} & \textbf{Perf. (\%)} & \textbf{Fair. (\%)} & \textbf{Perf. (\%)} \\
\midrule
  \multicolumn{5}{c}{ACSIncome dataset} \\
\midrule

FairGBM & $99.6 \pm 0.73$ & $81.6 \pm 0.08$ & $99.4 \pm 0.74$ & $81.7 \pm 0.09$ \\
LightGBM & $75.6 \pm 3.28$ & $80.8 \pm 0.80$ & $75.5 \pm 3.32$ & $80.8 \pm 0.80$ \\
GS & $66.4 \pm 1.49$ & $81.7 \pm 0.19$ & $65.9 \pm 1.36$ & $81.8 \pm 0.20$ \\
RS & $42.3 \pm 25.8$ & $77.0 \pm 3.70$ & $42.4 \pm 25.8$ & $77.0 \pm 3.73$ \\
EG & $94.4 \pm 0.32$ & $81.6 \pm 0.16$ & $93.8 \pm 0.11$ & $81.6 \pm 0.18$ \\

\midrule
  \multicolumn{5}{c}{AOF dataset} \\
\midrule

FairGBM & $92.2 \pm 4.19$ & $64.8 \pm 2.54$ & $90.1 \pm 4.51$ & $64.7 \pm 2.59$ \\
LightGBM & $70.2 \pm 7.92$ & $55.8 \pm 3.97$ & $78.4 \pm 9.89$ & $55.8 \pm 3.36$ \\
GS & $98.9 \pm 0.82$ & $23.4 \pm 3.71$ & $98.7 \pm 1.37$ & $23.4 \pm 3.87$ \\
RS & $95.3 \pm 3.55$ & $31.2 \pm 4.31$ & $96.1 \pm 3.47$ & $31.3 \pm 4.53$ \\

\bottomrule
\end{tabular}


==> tables-2022/results_bootstrapping_alpha=0.75.tex <==
\begin{tabular}{l|cccc}
\toprule
    \multirow{3}{*}{\textbf{Algorithm}} & \multicolumn{4}{c}{\textbf{Trade-off} $\alpha = 0.75$} \\
        & \multicolumn{2}{c}{\textbf{Validation}}  & \multicolumn{2}{c}{\textbf{Test}} \\
        & \textbf{Fair.} & \textbf{Perf.} & \textbf{Fair.} & \textbf{Perf.} \\
\midrule
  \multicolumn{5}{c}{ACSIncome dataset} \\
\midrule

FairGBM & $99.5 \pm 0.83$ & $81.7 \pm 0.06$ & $99.3 \pm 0.89$ & $81.7 \pm 0.08$ \\
LightGBM & $75.0 \pm 3.41$ & $81.1 \pm 0.87$ & $74.6 \pm 3.57$ & $81.1 \pm 0.88$ \\
GS & $66.4 \pm 1.53$ & $81.8 \pm 0.14$ & $65.8 \pm 1.39$ & $81.8 \pm 0.14$ \\
RS & $41.4 \pm 26.6$ & $77.5 \pm 3.04$ & $41.5 \pm 26.5$ & $77.5 \pm 3.06$ \\
EG & $94.4 \pm 0.33$ & $81.6 \pm 0.15$ & $93.8 \pm 0.13$ & $81.6 \pm 0.17$ \\

\midrule
  \multicolumn{5}{c}{AOF dataset} \\
\midrule

FairGBM & $89.3 \pm 4.62$ & $65.9 \pm 1.33$ & $87.5 \pm 3.36$ & $65.9 \pm 1.64$ \\
LightGBM & $58.0 \pm 9.39$ & $61.7 \pm 2.68$ & $66.6 \pm 14.9$ & $61.1 \pm 2.86$ \\
GS & $98.5 \pm 1.0$ & $23.6 \pm 3.45$ & $98.4 \pm 1.67$ & $23.7 \pm 3.64$ \\
RS & $84.0 \pm 19.3$ & $36.9 \pm 8.43$ & $84.6 \pm 20.9$ & $37.4 \pm 8.89$ \\

\bottomrule
\end{tabular}


==> tables-2022/results_bootstrapping_alpha=0.95.tex <==
\begin{tabular}{l|cccc}
\toprule
    \multirow{3}{*}{\textbf{Algorithm}} & \multicolumn{4}{c}{\textbf{Trade-off} $\alpha = 0.95$} \\
        & \multicolumn{2}{c}{\textbf{Validation}}  & \multicolumn{2}{c}{\textbf{Test}} \\
        & \textbf{Fair. (\%)} & \textbf{Perf. (\%)} & \textbf{Fair. (\%)} & \textbf{Perf. (\%)} \\
\midrule
  \multicolumn{5}{c}{ACSIncome dataset} \\
\midrule

FairGBM & $98.7 \pm 1.07$ & $81.8 \pm 0.06$ & $98.5 \pm 1.22$ & $81.8 \pm 0.06$ \\
LightGBM & $71.2 \pm 0.30$ & $81.9 \pm 0.04$ & $70.8 \pm 0.34$ & $82.0 \pm 0.05$ \\
GS & $66.3 \pm 1.54$ & $81.8 \pm 0.14$ & $65.8 \pm 1.40$ & $81.8 \pm 0.14$ \\
RS & $38.3 \pm 25.6$ & $77.8 \pm 2.96$ & $38.4 \pm 25.6$ & $77.8 \pm 2.97$ \\
EG & $94.4 \pm 0.36$ & $81.6 \pm 0.15$ & $93.9 \pm 0.13$ & $81.6 \pm 0.16$ \\

\midrule
  \multicolumn{5}{c}{AOF dataset} \\
\midrule

FairGBM & $80.0 \pm 9.79$ & $66.6 \pm 0.88$ & $80.2 \pm 9.13$ & $66.6 \pm 1.06$ \\
LightGBM & $33.7 \pm 1.70$ & $67.6 \pm 0.47$ & $36.0 \pm 1.29$ & $67.3 \pm 1.01$ \\
GS & $98.5 \pm 0.99$ & $23.6 \pm 3.44$ & $98.3 \pm 1.74$ & $23.8 \pm 3.51$ \\
RS & $81.5 \pm 21.2$ & $37.6 \pm 9.15$ & $82.2 \pm 23.2$ & $38.2 \pm 9.64$ \\

\bottomrule
\end{tabular}


==> tables-2022/results_hpo_runtimes_full.tex <==
\begin{tabular}{l|cc}

\toprule
    \multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{2}{|c}{\textbf{Run-time}} \\
        & \textbf{Total (h)} & \textbf{Relative} \\
\midrule
  \multicolumn{3}{c}{ACSIncome dataset} \\
\midrule
 FairGBM    
    % & $0.999$ & $0.817$ & $0.997$ & $0.817$ 
    % & $0.999$ & $0.817$ & $0.997$ & $0.817$
    % & $0.994$ & $0.817$ & $0.993$ & $0.818$
    & $9.9$ & x2.1 \\

 LightGBM   
    % & $0.819$ & $0.792$ & $0.818$ & $0.792$ 
    % & $0.776$ & $0.806$ & $0.774$ & $0.807$ 
    % & $0.712$ & $0.820$ & $0.706$ & $0.820$
    & $4.6$ & \textit{baseline} \\

 GS         
    % & $0.683$ & $0.819$ & $0.676$ & $0.820$ 
    % & $0.683$ & $0.819$ & $0.676$ & $0.820$ 
    % & $0.683$ & $0.819$ & $0.676$ & $0.820$
    & $43.8$ & x9.6 \\    %% > Fairlearn-GS-10x10 (Note: 10x10)

 RS         
    % & $0.787$ & $0.812$ & $0.793$ & $0.812$ 
    % & $0.787$ & $0.812$ & $0.793$ & $0.812$ 
    % & $0.787$ & $0.812$ & $0.793$ & $0.812$
    & $37.1$ & x8.1 \\    %% > Fairlearn-GS (Note: 100x1)

 EG         
    % & $0.949$ & $0.818$ & $0.939$ & $0.819$ 
    % & $0.949$ & $0.818$ & $0.939$ & $0.819$ 
    % & $0.949$ & $0.818$ & $0.939$ & $0.819$
    & $99.4$ & x21.7 \\    %% > Fairlearn-EG

\midrule

  \multicolumn{3}{c}{AOF dataset} \\
\midrule
 FairGBM    
    % & $0.952$ & $0.655$ & $0.915$ & $0.666$
    % & $0.904$ & $0.674$ & $0.876$ & $0.661$
    % & $0.904$ & $0.674$ & $0.876$ & $0.661$
    & $3.5$ & x2.4 \\

 LightGBM   
    % & $0.812$ & $0.519$ & $0.866$ & $0.526$ 
    % & $0.635$ & $0.617$ & $0.774$ & $0.595$ 
    % & $0.319$ & $0.682$ & $0.357$ & $0.672$
    & $1.4$ & \textit{baseline} \\

 GS         
    % & $0.988$ & $0.277$ & $0.999$ & $0.284$ 
    % & $0.988$ & $0.277$ & $0.999$ & $0.284$ 
    % & $0.988$ & $0.277$ & $0.999$ & $0.284$
    & $21.4$ & x14.7 \\

 RS         
    % & $0.922$ & $0.357$ & $0.935$ & $0.359$ 
    % & $0.888$ & $0.381$ & $0.889$ & $0.389$ 
    % & $0.377$ & $0.547$ & $0.336$ & $0.563$
    & $10.3$ & x7.1 \\

\bottomrule
\end{tabular}

